Order-Invariant Cardinality Estimators Are Differentially Private

We consider privacy in the context of streaming algorithms for cardinality estimation. We show that a large class of algorithms all satisfy $\epsilon$-differential privacy, so long as (a) the algorithm is combined with a simple down-sampling procedure, and (b) the cardinality of the input stream is $\Omega(k/\epsilon)$. Here, $k$ is a certain parameter of the sketch that is always at most the sketch size in bits, but is typically much smaller. We also show that, even with no modification, algorithms in our class satisfy $(\epsilon, \delta)$-differential privacy, where $\delta$ falls exponentially with the stream cardinality. Our analysis applies to essentially all popular cardinality estimation algorithms, and substantially generalizes and tightens privacy bounds from earlier works.

==> space-ratio.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkturquoise23190207}{RGB}{23,190,207}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{axis}[
width=10cm, height=4cm,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  anchor=north west,
  at={(0.0,1.25)},
  legend columns=2,
  draw=none
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Number of buckets: \(\displaystyle k\)},
xtick={128, 256, 512, 1024, 2048, 4096},
xticklabels={
\(\hspace*{-0.5em}\displaystyle 2^7\),
\(\hspace*{0.125em}\displaystyle 2^8\),
\(\displaystyle 2^9\),
\(\displaystyle 2^{10}\),
\(\displaystyle 2^{11}\),
\(\displaystyle 2^{12}\),
},
xmajorgrids,
xmin=-70.4, xmax=4294.4,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Space Ratio: $r$},
ymajorgrids,
ymin=0.963671440825121, ymax=1.76289974267245,
ytick style={color=black}
]
\addplot [semithick, black, fill opacity=0.1, mark=*, mark size=2, mark options={solid}, forget plot, draw opacity = 0.0]
table {%
128 1.11231719189046
128 1.17712806172517
128 1.08254642014359
128 1.03910143462217
128 1.11231719189046
128 1.11715300223093
128 1.11934290006491
128 1.17673353691285
128 1.16626197003318
128 1.10017737402625
128 1.13169419836934
128 1.06625415720949
128 1.14361202721876
128 1.16818774479176
128 1.11231719189046
128 1.13534757818233
128 1.12403096221669
128 1.01218459962024
128 1.08254642014359
128 1.11934290006491
128 1.1402813001478
128 1.14361202721876
128 1.13169419836934
128 1.14629308993999
128 1.08937223632371
128 1.09449169067938
128 1.13169419836934
128 1.06625415720949
128 1.07015027961422
128 1.22003701253396
128 1.10017737402625
128 1.04850474159853
128 1.15286364152708
128 1.08757934304865
128 1.07392825439757
128 1.14361202721876
128 1.10601774132577
128 1.12403096221669
128 1.10017737402625
128 1.06625415720949
128 1.13835124348476
128 1
128 1.13169419836934
128 1.07801965209338
128 1.17704456683319
128 1.07015027961422
128 1.11231719189046
128 1.16500440498265
128 1.08053147863426
128 1.11231719189046
128 1.13169419836934
128 1.09449169067938
128 1.15286364152708
128 1.08757934304865
128 1.08937223632371
128 1.06625415720949
128 1.11715300223093
128 1.09449169067938
128 1.08254642014359
128 1
128 1.16500440498265
128 1.04610926708375
128 1.07015027961422
128 1.14361202721876
128 1.13534757818233
128 1
128 1.11094792656576
128 1.11934290006491
128 1.15286364152708
128 1.13534757818233
128 1.15286364152708
128 1.10017737402625
128 1.08254642014359
128 1.11094792656576
128 1.10601774132577
128 1.13835124348476
128 1.17612198783612
128 1.1402813001478
128 1.13169419836934
128 1.11231719189046
128 1.07801965209338
128 1.11231719189046
128 1.07801965209338
128 1.05113791926663
128 1.08937223632371
128 1.15512578312118
128 1
128 1.01158355117549
128 1.08254642014359
128 1.10017737402625
128 1.05404457790014
128 1.09449169067938
128 1.1568910657988
128 1.20047344433045
128 1.08254642014359
128 1.13169419836934
128 1.09449169067938
128 1.12403096221669
128 1.13169419836934
128 1.13169419836934
};
\addplot [semithick, black, fill opacity=0.1, mark=*, mark size=2, mark options={solid}, forget plot, draw opacity = 0.0]
table {%
256 1.18749533823123
256 1.22292692123097
256 1.115137621273
256 1.21704642677655
256 1.17704456683319
256 1.20535401127832
256 1.14845846367979
256 1.16778514010492
256 1.19620800900369
256 1.13835124348476
256 1.18749533823123
256 1.18807803705661
256 1.17712806172517
256 1.19205119221557
256 1.12121912108788
256 1.17712806172517
256 1.26319353278819
256 1.22003701253396
256 1.19906233284066
256 1.14629308993999
256 1.1568910657988
256 1.19763409925189
256 1.16716289781076
256 1.19620800900369
256 1.15826393030397
256 1.1568910657988
256 1.13835124348476
256 1.18807803705661
256 1.16716289781076
256 1.27626470333318
256 1.14629308993999
256 1.17703811082297
256 1.10532364728752
256 1.13117422818559
256 1.17712806172517
256 1.13117422818559
256 1.12465859662611
256 1.20970859610513
256 1.13117422818559
256 1.18807803705661
256 1.20535401127832
256 1.16716289781076
256 1.13835124348476
256 1.19763409925189
256 1.20535401127832
256 1.13534757818233
256 1.18680433925142
256 1.16716289781076
256 1.18680433925142
256 1.09988114122372
256 1.12121912108788
256 1.12121912108788
256 1.16716289781076
256 1.16716289781076
256 1.19763409925189
256 1.115137621273
256 1.17712806172517
256 1.19620800900369
256 1.15826393030397
256 1.19906233284066
256 1.12465859662611
256 1.14845846367979
256 1.1934095082085
256 1.18603754332792
256 1.17712806172517
256 1.20970859610513
256 1.15932375324148
256 1.17703811082297
256 1.16716289781076
256 1.150210039214
256 1.21704642677655
256 1.06373026776682
256 1.16716289781076
256 1.17703811082297
256 1.19763409925189
256 1.20535401127832
256 1.17704456683319
256 1.12465859662611
256 1.16716289781076
256 1.14845846367979
256 1.18680433925142
256 1.1568910657988
256 1.13835124348476
256 1.1568910657988
256 1.14083212308679
256 1.17712806172517
256 1.22635175603689
256 1.14629308993999
256 1.2300660120196
256 1.17704456683319
256 1.24423079304798
256 1.13835124348476
256 1.20535401127832
256 1.15826393030397
256 1.15932375324148
256 1.12121912108788
256 1.2033288376318
256 1.17712806172517
256 1.1568910657988
256 1.13835124348476
};
\addplot [semithick, black, fill opacity=0.1, mark=*, mark size=2, mark options={solid}, forget plot, draw opacity = 0.0]
table {%
512 1.26939958502434
512 1.25397317359082
512 1.26319353278819
512 1.25755072422853
512 1.26939958502434
512 1.29223864398112
512 1.30923976252546
512 1.27069515636465
512 1.2210647294575
512 1.25551944307475
512 1.2315141403621
512 1.25551944307475
512 1.28519886494287
512 1.3162436037847
512 1.22767024869695
512 1.31701483706065
512 1.40481687155078
512 1.28519886494287
512 1.26939958502434
512 1.26939958502434
512 1.27739108954411
512 1.32461901692393
512 1.25551944307475
512 1.2455822460565
512 1.20906195512217
512 1.30029571798868
512 1.24766477007279
512 1.31474995348819
512 1.2455822460565
512 1.31895755620841
512 1.30128593507683
512 1.30759972577188
512 1.25551944307475
512 1.27830238657094
512 1.30586536052072
512 1.27739108954411
512 1.2780318956697
512 1.25906400731646
512 1.26319353278819
512 1.22792368174378
512 1.29223864398112
512 1.18349163245035
512 1.22767024869695
512 1.26319353278819
512 1.21810429198553
512 1.13979804568941
512 1.25033156024851
512 1.34647741678164
512 1.32461901692393
512 1.2455822460565
512 1.30923976252546
512 1.27739108954411
512 1.19779673126353
512 1.28519886494287
512 1.30923976252546
512 1.2780318956697
512 1.25033156024851
512 1.2780318956697
512 1.25033156024851
512 1.33205965329266
512 1.24295015435916
512 1.23539904619854
512 1.31895755620841
512 1.21810429198553
512 1.28519886494287
512 1.23539904619854
512 1.2455822460565
512 1.26461462527077
512 1.20919388027897
512 1.2780318956697
512 1.26461462527077
512 1.2780318956697
512 1.27739108954411
512 1.30759972577188
512 1.32861405283244
512 1.32175274327213
512 1.22424382421758
512 1.31701483706065
512 1.29283116977618
512 1.2780318956697
512 1.30029571798868
512 1.24295015435916
512 1.22424382421758
512 1.22767024869695
512 1.26319353278819
512 1.27069515636465
512 1.29223864398112
512 1.29782052831117
512 1.30029571798868
512 1.36031831268176
512 1.33533948590689
512 1.32861405283244
512 1.31474995348819
512 1.32175274327213
512 1.33205965329266
512 1.17608757365641
512 1.32861405283244
512 1.30923976252546
512 1.29314494167488
512 1.2964342113382
};
\addplot [semithick, black, fill opacity=0.1, mark=*, mark size=2, mark options={solid}, forget plot, draw opacity = 0.0]
table {%
1024 1.36084880671453
1024 1.38106803460942
1024 1.41073113960734
1024 1.37767130309975
1024 1.42226474948867
1024 1.38826927895855
1024 1.44770528688221
1024 1.42290425159787
1024 1.45669735521449
1024 1.46490031707173
1024 1.30044489420224
1024 1.33368799002272
1024 1.28713717204707
1024 1.39243156900933
1024 1.37767130309975
1024 1.41654600348098
1024 1.42676085025073
1024 1.31914637389584
1024 1.32458373639409
1024 1.36111543741802
1024 1.46234477367664
1024 1.29351926796131
1024 1.41654600348098
1024 1.32136576918028
1024 1.39344470356937
1024 1.37224340788517
1024 1.36672579134208
1024 1.40710497167934
1024 1.36084880671453
1024 1.41337947385202
1024 1.34960366903484
1024 1.36084880671453
1024 1.37767130309975
1024 1.37111397773671
1024 1.36028303811315
1024 1.33368799002272
1024 1.37224340788517
1024 1.38826927895855
1024 1.38482660797408
1024 1.38301234825511
1024 1.43342624182269
1024 1.46275642631952
1024 1.30226347631096
1024 1.40481687155078
1024 1.41245348019983
1024 1.37767130309975
1024 1.40850627488493
1024 1.39344470356937
1024 1.37767130309975
1024 1.28713717204707
1024 1.43919181111439
1024 1.37767130309975
1024 1.30580517145327
1024 1.36602149218172
1024 1.37224340788517
1024 1.40167088339982
1024 1.40356087775585
1024 1.33519175078333
1024 1.36111543741802
1024 1.33519175078333
1024 1.41073113960734
1024 1.41245348019983
1024 1.43800110464368
1024 1.43887479940879
1024 1.34482325092788
1024 1.43887479940879
1024 1.36084880671453
1024 1.37767130309975
1024 1.35540917537645
1024 1.37224340788517
1024 1.34036810846456
1024 1.43342624182269
1024 1.37904281204875
1024 1.37767130309975
1024 1.40356087775585
1024 1.39344470356937
1024 1.41654600348098
1024 1.39614843209863
1024 1.27711477168947
1024 1.37224340788517
1024 1.35025244459925
1024 1.33368799002272
1024 1.3790209405854
1024 1.35559335477626
1024 1.35540917537645
1024 1.36111543741802
1024 1.41245348019983
1024 1.43800110464368
1024 1.39344470356937
1024 1.36507594730436
1024 1.43304301261853
1024 1.35541805240316
1024 1.38826927895855
1024 1.37111397773671
1024 1.31626279649254
1024 1.42291749989537
1024 1.38106803460942
1024 1.36111543741802
1024 1.32216193937633
1024 1.45713987333608
};
\addplot [semithick, black, fill opacity=0.1, mark=*, mark size=2, mark options={solid}, forget plot, draw opacity = 0.0]
table {%
2048 1.46306929489549
2048 1.47800180894546
2048 1.44742544599521
2048 1.39042346155377
2048 1.43726633442498
2048 1.44105018402902
2048 1.49576066025178
2048 1.55296160691776
2048 1.55965685290409
2048 1.48877191279384
2048 1.49075675355877
2048 1.48396617602991
2048 1.3979156721848
2048 1.56060963825287
2048 1.50480849839098
2048 1.43931494160726
2048 1.54711054427144
2048 1.49662440907904
2048 1.45922762842647
2048 1.47904298323255
2048 1.52060777830951
2048 1.45140681278764
2048 1.42167220961265
2048 1.45534049739391
2048 1.47062040305611
2048 1.4829934222459
2048 1.36357262734399
2048 1.53705184959461
2048 1.53049974430165
2048 1.56817180377255
2048 1.47904298323255
2048 1.45922762842647
2048 1.41311592167307
2048 1.54905222909359
2048 1.55682730362878
2048 1.42956322162307
2048 1.4668665480403
2048 1.54509817169858
2048 1.48163122420273
2048 1.4829934222459
2048 1.3479584812935
2048 1.59016072679819
2048 1.47525740984566
2048 1.49245720008655
2048 1.54109840164496
2048 1.50480849839098
2048 1.48163122420273
2048 1.45214322917351
2048 1.47800180894546
2048 1.3979156721848
2048 1.44212945891501
2048 1.44479028872687
2048 1.47904298323255
2048 1.48689765623451
2048 1.42564177417767
2048 1.47904298323255
2048 1.47800180894546
2048 1.4668665480403
2048 1.47062040305611
2048 1.42621860267767
2048 1.42564177417767
2048 1.51280000291075
2048 1.46636597896892
2048 1.54109840164496
2048 1.44589113194206
2048 1.51280000291075
2048 1.52824008314281
2048 1.50480849839098
2048 1.54222337743596
2048 1.62625459958611
2048 1.50882775561816
2048 1.38741236432674
2048 1.57915609955659
2048 1.53295740824302
2048 1.50207336952441
2048 1.58980236282106
2048 1.47099902289878
2048 1.52462022756263
2048 1.42956322162307
2048 1.41689027328466
2048 1.47062040305611
2048 1.52060777830951
2048 1.4094626303033
2048 1.50074110520285
2048 1.53937627005482
2048 1.47504523244806
2048 1.51280000291075
2048 1.48522097292548
2048 1.49457174594795
2048 1.50576189545983
2048 1.56065028458492
2048 1.47433184072329
2048 1.51280000291075
2048 1.47062040305611
2048 1.47904298323255
2048 1.52361685714088
2048 1.55015886685483
2048 1.39354358565519
2048 1.51301888128207
2048 1.53049974430165
};
\addplot [semithick, black, fill opacity=0.1, mark=*, mark size=2, mark options={solid}, forget plot, draw opacity = 0.0]
table {%
4096 1.61439056141487
4096 1.49750466556205
4096 1.60852321338828
4096 1.63493909091561
4096 1.56417764434633
4096 1.58965271257306
4096 1.65312797612588
4096 1.57521931393051
4096 1.5867873885362
4096 1.59111558070201
4096 1.59249365057778
4096 1.55417504522264
4096 1.60379896107369
4096 1.69710860377658
4096 1.51879531800908
4096 1.60852321338828
4096 1.71215342000859
4096 1.60904951625951
4096 1.56135823871967
4096 1.60852321338828
4096 1.57249349962484
4096 1.61734509306962
4096 1.62938562779907
4096 1.54612030252744
4096 1.57249349962484
4096 1.57249349962484
4096 1.60087421293734
4096 1.62023552134072
4096 1.52847801329198
4096 1.67323870839082
4096 1.61148937435495
4096 1.58590184045834
4096 1.53988921834816
4096 1.65635847004911
4096 1.5779226932962
4096 1.54612030252744
4096 1.62594360985445
4096 1.62023552134072
4096 1.66770297019288
4096 1.55417504522264
4096 1.61702937516231
4096 1.72657118349757
4096 1.63742094770674
4096 1.56135823871967
4096 1.60362162104493
4096 1.60087421293734
4096 1.59624785291307
4096 1.62876207641919
4096 1.61173072104144
4096 1.54063685848889
4096 1.63980770919871
4096 1.56974487489249
4096 1.68670251841573
4096 1.52420102350446
4096 1.55564576884381
4096 1.45900839205736
4096 1.63155734546527
4096 1.68405134639101
4096 1.60904951625951
4096 1.58851905541148
4096 1.56697305474057
4096 1.62023552134072
4096 1.59111558070201
4096 1.58965271257306
4096 1.63742094770674
4096 1.64759910962597
4096 1.63432979573403
4096 1.60852321338828
4096 1.64462933811891
4096 1.70172835285408
4096 1.5867873885362
4096 1.58210351427188
4096 1.65312797612588
4096 1.53223338723438
4096 1.58060400401279
4096 1.63742094770674
4096 1.57507361820998
4096 1.55943557500091
4096 1.66770297019288
4096 1.61148937435495
4096 1.54882756061166
4096 1.62594360985445
4096 1.60553091850817
4096 1.66490152771043
4096 1.61702937516231
4096 1.58931977152194
4096 1.61734509306962
4096 1.61439056141487
4096 1.62991932413027
4096 1.51674006260533
4096 1.60904951625951
4096 1.60087421293734
4096 1.5671693804126
4096 1.59810400450184
4096 1.59531061413636
4096 1.62738084649249
4096 1.68405134639101
4096 1.66770297019288
4096 1.6451986679751
4096 1.69194468319235
};
\addplot [semithick, black]
table {%
128 1.10687014423058
256 1.16994790251659
512 1.27418320370432
1024 1.37914646272483
2048 1.48467408010395
4096 1.60402218212784
};
\addlegendentry{Mean space ratio}
\addplot [thick, darkturquoise23190207, dashed]
table {%
128 1.08489884608926
256 1.18595530256447
512 1.28701175903968
1024 1.38806821551488
2048 1.48912467199009
4096 1.59018112846529
};
\addlegendentry{ $r(k) = 0.10 \cdot \log_2(k) + 0.38$}
\end{axis}

\end{tikzpicture}

